Balancing Rates and Variance via Adaptive Batch-Size for Stochastic Optimization Problems

Stochastic gradient descent is a canonical tool for addressing stochastic optimization problems, and forms the bedrock of modern machine learning and statistics. In this work, we seek to balance the fact that attenuating step-size is required for exact asymptotic convergence with the fact that constant step-size learns faster in finite time up to an error. To do so, rather than fixing the mini-batch and the step-size at the outset, we propose a strategy to allow parameters to evolve adaptively. Specifically, the batch-size is set to be a piecewise-constant increasing sequence where the increase occurs when a suitable error criterion is satisfied. Moreover, the step-size is selected as that which yields the fastest convergence. The overall algorithm, two scale adaptive (TSA) scheme, is developed for both convex and non-convex stochastic optimization problems. It inherits the exact asymptotic convergence of stochastic gradient method. More importantly, the optimal error decreasing rate is achieved theoretically, as well as an overall reduction in computational cost. Experimentally, we observe that TSA attains a favorable tradeoff relative to standard SGD that fixes the mini-batch and the step-size, or simply allowing one to increase or decrease respectively.

==> Problemanalysis.tex <==
%!TEX root = mainOp.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Rotational Neural Networks  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The problem we considered here is 
\begin{equation}
\begin{split}
min_x F(x) = min_x \mathbb{E}_\xi [f(x,\xi)]
\end{split}
\end{equation}
where $\xi$ si a random variable and $f(x,\xi):\mathbb{R}^p \to \mathbb{R}$. For simplicity, we use the following notions:
\begin{equation}
\begin{split}
&f_i(x) = f(x,\xi_i)\\
&\nabla F(x) = \nabla \mathbb{E}_\xi [f(x,\xi)] = \mathbb{E}_\xi [\nabla f(x,\xi)]\\
&\nabla F_S(x)=\frac{1}{\vert S \vert}\sum_{i\in S}\nabla f_i(x)\\
&F_S(x) = \frac{1}{\vert S \vert}\sum_{i\in S} f_i(x)
\end{split}
\end{equation}

According to the Taylor's theorem, we have
\begin{equation}
\begin{split}
&F(x_{k+1})-F(x_k)\\
&\le \nabla F(x_k)^\perp (x_{k+1}-x_k)+\frac{\nabla^2F(x_k)}{2}\parallel x_{k+1}-x_k\parallel^2
\end{split}
\end{equation}
Based on the Lipschitz continuity with factor $M$, we have
\begin{equation}
\begin{split}
\nabla^2F(x_{k+1}) &= lim_{\triangle x_k \to 0}\frac{\nabla F(x_k+\triangle x_k)-\nabla F(x_k)}{\triangle x_k}\\
&\le M \frac{\triangle x_k}{\triangle x_k}\\
&=M
\end{split}
\end{equation}
So Eq. (3) can be derived to 
\begin{equation}
\begin{split}
&F(x_{k+1})-F(x_k)\\
&\le \nabla F(x_k)^\top (x_{k+1}-x_k)+\frac{M}{2}\parallel x_{k+1}-x_k\parallel^2
\end{split}
\end{equation}
Then for the first order method, we have
\begin{equation}
\begin{split}
x_{k+1} = x_k - \alpha_k \nabla F_{S_k}(x_k)
\end{split}
\end{equation}
where $\alpha_k$ is the stepsize in iteration $k$ and $S_k$ is the sample size in iteration $k$. Both of them can be different with regards to different iterations. Then substitute it into Eq. (5), we can get
\begin{equation}
\begin{split}
&F(x_{k+1})-F(x_k)\\
&\le -\alpha_k \nabla F(x_k)^\perp \nabla F_{S_k}(x_k)+\frac{\alpha_k^2 M}{2}\parallel \nabla F_{S_k}(x_k) \parallel^2
\end{split}
\end{equation}
Since $\mathbb{E}_{S_k}\left[ \nabla F_{S_k}(x_k)\right] = \nabla F(x_k)$, we can put expectation on both sides of Eq. (5) and get
\begin{equation}
\begin{split}
&\mathbb{E}_{S_k}\left[ F(x_{k+1})\right]\\
&\le \mathbb{E}_{S_k}\left[ F(x_{k})\right]-\alpha_k \parallel \nabla F(x_k)\parallel^2+\frac{\alpha_k^2 M}{2}\mathbb{E}_{S_k}\left[\parallel \nabla F_{S_k}(x_k)\parallel^2\right]
\end{split}
\end{equation}
Then we let $x^*$ represent the optimal solution for our problem. By adding $F(x^*)$ to both sides of Eq. (8), we can get
\begin{equation}
\begin{split}
&\mathbb{E}_{S_k}\left[ F(x_{k+1})-F(x^*)\right]\\
&\le \mathbb{E}_{S_k}\left[ F(x_{k})-F(x^*)\right]-\alpha_k \parallel \nabla F(x_k)\parallel^2\\
&+\frac{\alpha_k^2 M}{2}\mathbb{E}_{S_k}\left[\parallel \nabla F_{S_k}(x_k) - \nabla F(x_k)+\nabla F(x_k)\parallel^2\right]\\
& = \mathbb{E}_{S_k}\left[ F(x_{k})-F(x^*)\right]-\alpha_k \parallel \nabla F(x_k)\parallel^2\\
&+\frac{\alpha_k^2 M}{2} \left( \parallel \nabla F(x_k) \parallel^2 +\mathbb{E}_{S_k}\left[\parallel \nabla F_{S_k}(x_k)-\nabla F(x_k)\parallel^2\right]\right)\\
& = \mathbb{E}_{S_k}\left[ F(x_{k})-F(x^*)\right]-\left(\alpha_k-\frac{\alpha_k^2 M}{2}\right) \parallel \nabla F(x_k)\parallel^2\\
& + \frac{\alpha_k^2 M}{2}\mathbb{E}_{S_k}\left[\parallel \nabla F_{S_k}(x_k)-\nabla F(x_k)\parallel^2\right]
\end{split}
\end{equation}
Then consider the second term $\parallel \nabla F(x_k)\parallel^2$. Since we assume $F$ is strongly convex, so
\begin{equation}
\begin{split}
F(y)\ge F(z)+\nabla F(z)^\perp (y-z) + \frac{m}{2}\parallel y-z \parallel^2
\end{split}
\end{equation}
where $m$ is the parameter related to the strongly convex property. Note that the right side of Eq. (10) is a quadratic function with minimal value at $\hat{y}=z-\frac{1}{m}\nabla F(z)$. So we have
\begin{equation}
\begin{split}
F(y)&\ge F(z)+\nabla F(z)^\perp (\hat{y}-z) + \frac{m}{2}\parallel \hat{y}-z \parallel^2\\
&= F(z) - \frac{1}{2m}\parallel \nabla F(z) \parallel^2
\end{split}
\end{equation}
So let $y=x^*$ and $z=x_k$, we can get
\begin{equation}
\begin{split}
\parallel \nabla F(x_k) \parallel^2 \ge 2m(F(x_k)-F(x^*))
\end{split}
\end{equation}
Then we consider the third term $\mathbb{E}_{S_k}\left[\parallel \nabla F_{S_k}(x_k)-\nabla F(x_k)\parallel^2\right]$. Note that 
\begin{equation}
\begin{split}
\mathbb{E}_{S_k}\left[\parallel \nabla F_{S_k}(x_k)-\nabla F(x_k)\parallel^2\right] = \parallel Var(\nabla F_{S_k}(x_k)) \parallel_1
\end{split}
\end{equation}
Based on previous papers [], we have
\begin{equation}
\begin{split}
Var(\nabla F_{S_k}(x_k)) &= \frac{Var(\nabla f_i (x_k))}{\vert S_k \vert} \cdot \frac{N-\vert S_k \vert}{N-1}\\
& = \frac{Var(\nabla f_i(x_k))}{\vert S_k \vert}
\end{split}
\end{equation}
where $N$ is the total number of functions $f_i(x)$ in the problem, which we assume to be infinity.

With the assumption that $\parallel Var(\nabla f_i(x_k)) \parallel_1 \le w$, we can get
\begin{equation}
\begin{split}
\mathbb{E}_{S_k}\left[\parallel \nabla F_{S_k}(x_k)-\nabla F(x_k)\parallel^2\right] &= \parallel Var(\nabla F_{S_k}(x_k)) \parallel_1\\
&= \frac{\parallel Var(\nabla f_i(x_k)) \parallel_1}{\vert S_k \vert}\\
& \le \frac{w}{n_k}
\end{split}
\end{equation}
where $n_k$ is the number of sample size $S_k$. So substitute Eq. (12) and Eq. (15) into Eq. (9), we can have
\begin{equation}
\begin{split}
&\mathbb{E}_{S_k}\left[ F(x_{k+1})-F(x^*)\right]\\
& \le \left( 1-\alpha_km + \frac{Mm}{2}\alpha_k^2 \right) \mathbb{E}_{S_k}\left[ F(x_{k})-F(x^*)\right] + \frac{\alpha_k^2 M w}{2n_k}
\end{split}
\end{equation}
Then if we set $\alpha_k = \alpha$ and $n_k = n$ constants. According to the knowledge of geometrical sequences, we can derive
\begin{equation}
\begin{split}
&\mathbb{E}_{S_k}\left[ F(x_{k+1})-F(x^*)\right]\\
& \le \left( 1-\alpha m + \frac{Mm}{2}\alpha^2 \right)^{k+1} \mathbb{E}_{S_k}\left[ F(x_{0})-F(x^*)\right]\\
& + \frac{\alpha^2 M w}{2(\alpha m-\frac{Mm}{2}\alpha^2)n}\\
&= Q_1+Q_2
\end{split}
\end{equation}
Now we can see that the upper bound in Eq. (17) consists of two terms $Q_1$ and $Q_2$. For term $Q_1$, as long as $1-\alpha m + \frac{Mm}{2}\alpha^2 <1$, it is always decreasing. As for the second term $Q_2$, it is a function of stepsize $\alpha$ and sample size $n$. In other words, it is a constant since we have assumed that $\alpha$ and $n$ are constants here.





==> conclusions.tex <==
%!TEX root = mainStabilitySO3.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Conclusions   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> proofsStabilitySO31.tex <==
%!TEX root = mainOp.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Stability   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Permutation Equivariance of Graph Filters  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\title{Balancing Rates and Variance via Adaptive Batch-Sizes for Stochastic Optimization Problems
}


\section{Proof of Proposition 1} \label{pr:prop1}

\begin{proof}

From the truncated Taylor's expansion and Lipschitz continuity of $\nabla F(\bbx)$ in Assumption \ref{asm1}, we upper bound $F(\bbx_{k+1})$ as 
\begin{equation} \label{prprop11}
\begin{split}
F(\!\bbx_{k+1}\!)&\!\le\! F(\!\bbx_k\!) \!+\!\! \nabla F(\!\bbx_k\!)^\top\!\! \big(\!\bbx_{k+1}\!-\!\!\bbx_k\!\big)\!\!+\!\!\frac{L}{2} \| \bbx_{k\!+\!1}\!\!-\!\!\bbx_k \|^2_2.
\end{split}
\end{equation}
By substituting the update rule \eqref{eq:sgd} of SGD into \eqref{prprop11}, we get
\begin{equation} \label{prprop12}
\begin{split}
F(\!\bbx_{k\!+\!1}\!)&\!\le\!\! F(\!\bbx_k\!) \!-\!\! \alpha_k\! \nabla\! F(\!\bbx_k\!)^\top\! \nabla\! f_{S_k}\!(\!\bbx_k\!)\!\!+\!\!\frac{\alpha_k^2 L}{2}\|\! \nabla\! f_{S_k}\!(\!\bbx_k\!)\! \|^2_2.
\end{split}
\end{equation}
Take the expectation for both sides of \eqref{prprop12}, and by using the fact $\mathbb{E}\left[ \nabla f_{S_k}(\bbx_k)\right] = \mathbb{E}\left[\nabla F(\bbx_k)\right]$, we have
\begin{align}\label{prprop13}
&\mathbb{E}\!\left[ F(\bbx_{k+1})\right] \\
&\le\! \mathbb{E}\left[ F(\bbx_{k})\right] \!-\!\alpha_k \mathbb{E}\!\left[\| \nabla\! F(\bbx_k)\|^2_2 \right]\!+\!\frac{\alpha_k^2 L}{2}\mathbb{E}\!\left[\| \nabla\! f_{S_k}(\bbx_k)\|^2_2 \right]\nonumber
\end{align}
where the linearity of expectation is used. By subtracting $F(\bbx^*)$ in both sides of \eqref{prprop13}, we get
\begin{align} \label{prprop135}
&\mathbb{E}\left[ F(\bbx_{k+1})\!-\!F(\bbx^*)\right]\\
&\!\le\! \mathbb{E}\!\left[ F(\!\bbx_{k}\!)\!-\!\!F(\!\bbx^*\!)\right]\!-\!\alpha_k \mathbb{E}\!\left[\| \nabla\! F(\!\bbx_k\!)\|^2_2 \right]\!\!+\!\frac{\alpha_k^2 L}{2}\mathbb{E}\!\left[\| \nabla\! f_{S_k}\!(\!\bbx_k\!)\|^2_2 \right]\!.\nonumber
\end{align}

Consider the third term $\mathbb{E}\left[\parallel \nabla f_{S_k}(\bbx_k)\parallel^2\right]$ in the bound of \eqref{prprop135}. Note that for any random variable $x$, its variance is
\begin{equation}\label{prprop15}
\begin{split}
{\rm Var}[x]  = \mathbb{E}[x^2] - \mathbb{E}[x] \mathbb{E}[x].
\end{split}
\end{equation}
We then have
\begin{align} \label{prprop16}
\mathbb{E}\!\left[\| \nabla\! f_{S_k}\!(\!\bbx_k\!)\|^2_2\right] &\!\!=\! \mathbb{E}\!\left[\| \nabla\! F(\!\bbx_k\!) \|^2_2\right] \!\!+\!\mathbb{E}\!\left[\| \nabla\! f_{S_k}\!(\!\bbx_k\!)\!-\!\!\nabla\! F(\!\bbx_k\!)\|^2_2\right]\nonumber \\
&\!\!=\! \mathbb{E}\!\left[\| \nabla\! F(\bbx_k) \|^2_2\right] \!+\! \| {\rm Var}\! \left[ \nabla\! f_{S_k}\!(\bbx_k)\right] \|_1.
\end{align}
From \cite{Freund1962}, we proceed to estimate the variance vector ${\rm Var} \left[\nabla f_{S_k}(\bbx_k) \right]$ by
\begin{equation} \label{prprop17}
\begin{split}
{\rm Var}[\nabla f_{S_k}(\bbx_k)] = \frac{{\rm Var} \left[\nabla f_i (\bbx_k) \right]}{\vert S_k \vert} \cdot \frac{N-\vert S_k \vert}{N-1}
\end{split}
\end{equation}
where ${\rm Var} \left[\nabla f_i (\bbx_k) \right]$ is the population variance vector and $N$ is the number of samples drawn to approximate the distribution $\bbp$, which should be large enough and usually assumed to be infinity. By substituting \eqref{prprop17} into $\| {\rm Var} \left[ \nabla f_{S_k}(\bbx_k)\right] \|_1$ with $\vert S_k \vert = n_k$, we have
\begin{equation} \label{prprop18}
\begin{split}
\| {\rm Var} \left[ \nabla f_{S_k}(\bbx_k)\right] \|_1 \le \| \frac{{\rm Var}[\nabla f_i(\bbx_k)]}{n_k} \|_1 \le \frac{w}{n_k}
\end{split}
\end{equation}
where the last inequality is due to Assumption 2. By substituting \eqref{prprop18} into \eqref{prprop16} and then into \eqref{prprop135}, we get
\begin{align} \label{prprop19}
&\mathbb{E}\left[ F(\bbx_{k+1})-F(\bbx^*)\right] \\
&\!\!\le\! \mathbb{E}\!\left[ F(\bbx_{k})\!-\!F(\bbx^*)\right] \!-\! \left(\! \alpha_k \!-\! \frac{L\alpha_k^2}{2}\! \right)\! \mathbb{E}\!\left[\| \nabla\! F(\bbx_k) \|^2_2\right] \!+\! \frac{\alpha_k^2 L w}{2n_k}.\nonumber
\end{align}

Now consider the term $\| \nabla F(\bbx_k)\|^2_2$. From Assumption 1, it holds that for any $ \bbx,\bby \in \mathbb{R}^p$,
\begin{equation} \label{prprop14}
\begin{split}
F(\bbx)\ge F(\bby)+\nabla F(\bby)^\top (\bbx-\bby) + \frac{\ell}{2}\| \bbx-\bby \|^2_2.
\end{split}
\end{equation}
Since the right side of \eqref{prprop14} is a quadratic function with minimal value at $\widehat{\bbx}=\bby-\frac{1}{\ell}\nabla F(\bby)$, we have
\begin{equation}
\begin{split}
F(\bbx)&\ge F(\bby)+\nabla\! F(\bby)^\top (\widehat{\bbx}-\bby) + \frac{\ell}{2}\| \widehat{\bbx}-\bby\|^2_2 \\
&= F(\bby) - \frac{1}{2\ell}\| \nabla F(\bby) \|^2_2.
\end{split}
\end{equation}
Then let $\bbx=\bbx^*$ and $\bby=\bbx_k$, and we get
\begin{equation} \label{prprop145}
\begin{split}
\| \nabla F(\bbx_k) \|^2_2 \ge 2\ell\left(F(\bbx_k)-F(\bbx^*)\right).
\end{split}
\end{equation}

By substituting \eqref{prprop145} into \eqref{prprop19}, we obtain
\begin{equation} \label{prprop110}
\begin{split}
&\mathbb{E}\left[ F(\bbx_{k+1})-F(\bbx^*)\right]\\
& \le \left( 1-2\alpha_k \ell + L\ell\alpha_k^2 \right) \mathbb{E}\left[ F(\bbx_{k})-F(\bbx^*)\right] + \frac{\alpha_k^2 L w}{2n_k}.
\end{split}
\end{equation}
Observe that \eqref{prprop110} is a recursion process such that we can continue deriving the bound until it is represented by the initial condition $F(\bbx_{0})-F(\bbx^*)$ as
\begin{align}
\mathbb{E}\!\left[ F\!(\!\bbx_{k\!+\!1}\!)\!-\!F(\!\bbx^*\!)\right] &\!\le\!\! \big(\! \prod_{i
=0}^k\! 1\!\!-\!2\alpha_i \ell \!+\! L\ell\alpha_i^2 \big) \big( F(\bbx_{0})\!-\!F(\bbx^*)\big)\nonumber\\
&\!\! +\! \sum_{i=0}^k\! \big( \frac{\alpha_i^2 L w}{2n_i}\! \prod_{j=i+1}^k\! 1\!-\!2\alpha_j \ell \!+\! L\ell\alpha_j^2 \big).
\end{align}
Let $r(\alpha) = 1-2\alpha \ell + L\ell\alpha^2$ and we complete the proof.


\end{proof}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Corollary 1} \label{pr:coro11}

\begin{proof}
By substituting $\alpha_k = \alpha$ and $n_k = n$ into Proposition \ref{prop1}, we have
\begin{equation}\label{pr:coroeq1}
\begin{split}
 &\mathbb{E}\left[ F(\bbx_{k+1})-F(\bbx^*)\right] \\
 &\le r(\alpha)^{k+1} \left( F(\bbx_{0})\!-\!F(\bbx^*) \right) \!+\! \sum_{i=0}^k \left( \frac{\alpha^2 L w}{2n} r(\alpha)^{k-i} \right).
\end{split}
\end{equation}
Note that the second term in \eqref{pr:coroeq1} is a geometric series with the common ratio $r(\alpha)$. By summing terms up, we have
 \begin{equation}\label{pr:coroeq2}
\begin{split}
\sum_{i=0}^k \left( \frac{\alpha^2 L w}{2n} r(\alpha)^{k-i} \right) &= \frac{\alpha^2 L w}{2n} \cdot \frac{1-r(\alpha)^{k+1}}{1-r(\alpha)} \\
& \le \frac{\alpha^2 L w}{2n (1-r(\alpha))},
\end{split}
\end{equation}
where $r(\alpha) < 1$ is used in the last inequality. By substituting $r(\alpha) = 1-2\alpha \ell + L\ell\alpha^2$ into \eqref{pr:coroeq2}, we complete the proof.
\end{proof}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Proposition 2} \label{pr:prop2}

\begin{proof}
From the Taylor expansion for $F(\bbx_{t+1})$ and the Lipschitz continuity of $ \nabla F(\bbx)$ in Assumption 1, we have
%
\begin{equation} \label{eq:prprop22}
\begin{split}
\!\!\mathbb{E}\!\left[ \!F\!(\!\bbx_{k\!+\!1}\!) \right] &\! \le \! \mathbb{E}\!\big[\! F\!(\!\bbx_{k}\!)\!\!+\!\! \nabla\! F(\!\bbx_{k}\!)^\top\! (\!\bbx_{k\!+\!1}\!\!-\!\bbx_k\!) \!\!+\!\! \frac{L}{2} \| \bbx_{k\!+\!1}\!\!-\!\!\bbx_k \|_2^2\! \big]\!.
\end{split}
\end{equation}
%
Substituting the update rule \eqref{eq:sgd} of SGD into \eqref{eq:prprop22}, we get
\begin{equation}\label{eq:prprop225}
\begin{split}
\!\!\mathbb{E}\!\left[ F(\!\bbx_{k\!+\!1}\!)\right] &\!\le\! \mathbb{E}\big[\! F(\!\bbx_{k}\!)\!\! -\! \alpha_k \!\nabla\! F(\!\bbx_{k}\!)^\top\! \nabla\! f_{S_k}\!(\!\bbx_k\!) \!+\!\! \frac{\alpha_k^2 L}{2} \| \nabla\! f_{S_k}\!(\!\bbx_k\!) \|_2^2\big]\!.
\end{split}
\end{equation}
%
With the linearity of expectation and the fact that $\mathbb{E}[\nabla f_{S_k}(\bbx_k)]=\mathbb{E}[\nabla F(\bbx_k)]$, \eqref{eq:prprop225} becomes
\begin{align}\label{eq:prprop23}
&\mathbb{E}\left[ F(\bbx_{k+1})\right] \\
&\le\! \mathbb{E}\left[ F(\bbx_{k}) \right] \!-\! \alpha_k \mathbb{E}\!\left[ \| \nabla\! F(\bbx_{k})\|_2^2 \right]\! +\!\frac{\alpha_k^2 L}{2} \mathbb{E}\left[ \| \nabla\! f_{S_k}\!(\bbx_k) \|_2^2\right]\!.\nonumber
\end{align}
Consider the term $\mathbb{E}\left[\| \nabla f_{S_k}(\bbx_k)\|_2^2\right]$ in the bound of \eqref{eq:prprop23}. By substituting \eqref{prprop18} in the proof of Proposition \ref{prop1} into \eqref{eq:prprop23}, we get
\begin{align}\label{eq:prprop27}
%\begin{split}
&\mathbb{E}\left[ F(\bbx_{k+1})\right] \\
%
&\le \mathbb{E}\left[ F(\bbx_{k})\right]-\big(\alpha_k-\frac{\alpha_k^2 L}{2}\big)
 \mathbb{E}\left[ \| \nabla F(\bbx_k)\|^2 \right] + \frac{\alpha_k^2 L w}{2 n_k.}\nonumber
%\end{split}
\end{align}

Here, we use $\parallel \nabla_\bbx F(\bbx_{t}) \parallel^2_2 \le \epsilon$ as the convergence criterion to judge the approximate stationary in non-convex optimization problems, where $\epsilon$ can be any small value. We then focus on the term $\mathbb{E}\left[ \| \nabla F(\bbx_{t})\|_2^2 \right]$ in the bound of \eqref{eq:prprop27} and move it to the left side as
\begin{align} \label{eq:prprop28}
%\begin{split}
&\mathbb{E}\left[ \| \nabla F(\bbx_{k})\|_2^2 \right] \\
&\le \frac{1}{\alpha_k-\frac{\alpha_k^2 L}{2}} \mathbb{E}[ F(\bbx_{k}) - F(\bbx_{k+1}) ]+ \frac{\alpha_k^2 L w}{2n_k \big( \alpha_k-\frac{\alpha_k^2 L}{2}\big)}\nonumber
%\end{split}
\end{align}
The bound in \eqref{eq:prprop28} cannot be used to show the convergence due to the existence of term $\mathbb{E}[ F(\bbx_{k}) - F(\bbx_{k+1}) ]$. To handle this issue, note that \eqref{eq:prprop28} holds for all iterations $k=0,1,\ldots$ and we have $\alpha_k = \alpha$ as a constant, such that we have
\begin{align}
%\begin{split}
&\!\!\sum_{i\!=\!0}^{k\!-\!1}\!\! \mathbb{E}\!\left[ \| \nabla\! F(\!\bbx_{i}\!)\|_2^2 \right] \!\!\le\!\! \frac{1}{\alpha\!\!-\!\frac{\alpha^2 L}{2}} \mathbb{E}[ F(\!\bbx_{0}\!) \!\!-\!\! F(\!\bbx_{k\!+\!1}\!) ]\!\!+\!\! \sum_{i\!=\!0}^{k\!-\!1}\!\! \frac{ \alpha L w}{2n_i\! \big(1\!\!-\!\frac{\alpha L}{2}\!\big)}.
%\end{split}
\end{align}
Thus, we have
\begin{align} \label{eq:prprop29}
&\min_{0 \le i \le {k-1}} \mathbb{E}\left[ \| \nabla F(\bbx_{i})\|_2^2 \right] \le \frac{1}{k} \sum_{i=0}^{k-1} \mathbb{E}\left[ \| \nabla F(\bbx_{i})\|_2^2 \right] \\
& \le \frac{1}{\alpha k-\frac{\alpha^2 L k}{2}} \left( F(\bbx_{0}) - F(\bbx^*) \right)+ \sum_{i=0}^{k-1} \frac{ \alpha L w}{2k n_i \left(1-\frac{\alpha L}{2}\right)}\nonumber
\end{align}
where the last inequality is due to the fact that $F(\bbx^*)=\min_{\bbx} F(\bbx) \le F(\bbx_{k+1})$ where $\bbx^*$ is an optimal solution of \eqref{eq:main_prob}. We then complete the proof.
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






